Dependency Smells in JavaScript Projects

Dependency management in modern software development poses many challenges for developers who wish to stay up to date with the latest features and fixes whilst ensuring backwards compatibility. Project maintainers have opted for varied, and sometimes conflicting, approaches for maintaining their dependencies. Opting for unsuitable approaches can introduce bugs and vulnerabilities into the project, introduce breaking changes, cause extraneous installations, and reduce dependency understandability, making it harder for others to contribute effectively. In this paper, we empirically examine evidence of recurring dependency management issues (dependency smells). We look at the commit data for a dataset of 1,146 active JavaScript repositories to catalog, quantify and understand dependency smells. Through a series of surveys with practitioners, we identify and quantify seven dependency smells with varying degrees of popularity and investigate why they are introduced throughout project history. Our findings indicate that dependency smells are prevalent in JavaScript projects with two or more distinct smells appearing in 80% of the projects, but they generally infect a minority of a project's dependencies. Our observations show that the number of dependency smells tend to increase over time. Practitioners agree that dependency smells bring about many problems including security threats, bugs, dependency breakage, runtime errors, and other maintenance issues. These smells are generally introduced as developers react to dependency misbehaviour and the shortcomings of the npm ecosystem.

==> Methodology_and_Data.tex <==


%We start by explaining how we curated the necessary data to create our dataset, followed by the methodology used to extract, parse, and analyze the information from the projects.


\section{Data Curation}
\label{sec:data-curation}

%An important aspect of any empirical study is the data. 

We curate a large set of open-source GitHub projects to create our dataset.
We chose to study projects written in JavaScript since it is the most popular programming language on Github~\cite{TheState18online}. We also study \npm since it is the official registry of JavaScript packages with more than 1.5 million packages.

We start our data collection by retrieving the GitHub metadata from GHTorrent~\cite{Ghtorrent2019} containing data until June 1st, 2019.
We use this metadata to then identify non-forked open-source Javascript projects that have a minimum of 10 contributing authors and at least 10 commits since January 2019, that is, six months before the data collection started. 
With this criteria, we aim at filtering projects that are actively maintained by at least a medium sized team of developers, akin to the high-quality software development project, and reduce the chances of skewing our results towards abandoned and toy projects, prevalent in the GitHub platform~\cite{Kalliamvakou:14:MiningGithub,abdalkareem2017}.

%In this study, we aim at analyzing open-source Javascript projects that have been 
%
%This study strictly focuses on open source projects which have an active and accessible online repository. We have first retrieved the entire GitHub metadata database up to 2019-06-01 (latest) from GHTorrent \cite{Ghtorrent2019}. We have then written Python scripts to filter a set of actively developed projects by applying the criteria in Table~\ref{tab:criteria}. We define active projects as the ones that have a minimum number of 10 contributing authors and a minimum number of 10 commits in the last six months of our dataset (i.e. 2018-12-01 to 2019-06-01). We believe that investigating bad smells in active projects (in terms of commits and collaboration) will provide a more meaningful outcome that is less affected by noisy projects in the ecosystem.

%\begin{table}
%  \caption{Criteria for selecting the projects}
%  \label{tab:criteria}
%  \begin{tabular}{l|l}
%    \toprule
%    Criteria & Value\\
%    \midrule
%    \texttt Source Control & GitHub\\
%    \texttt Language & JavaScript\\
%    \texttt  Authors & >=10 Authors from 2018-12-01 to 2019-06-01\\
%    \texttt Commits & >=10 Commits from 2018-12-01 to 2019-06-01\\
%    \bottomrule
%  \end{tabular}
%\end{table}

%Our selection criteria filtered a total 2,360 projects. We initially attempted to use Libraries.io \cite{Libraries2019} to retrieve the dependencies as their dataset includes every dependency in the ecosystem. However, this only includes repositories which have a corresponding entry in the \npm package manager. While this would still include the majority of our selected repositories, a considerable number of non-library software projects would be left out. More importantly, the dataset contains a history of dependencies for the libraries but only a current snapshot for the repositories. This alone negates the use of this dataset as we have to look at the history of the dependency constraints for the repositories in order to answer our research questions.

Using our selection criteria, we identified a total of 2,216 project candidates. 
We further prune this dataset by 1) removing 569 projects that do not contain any package.json, making it impossible to reliably pinpoint their dependencies and therefore, their dependency smells, and 2) removing 413 projects that had no runtime dependencies in their package.json, as development and optional dependencies are out of the scope of this study.
We were left with 1,146 projects as our dataset. This accounts for 26,924 dependency constraints (in the latest snapshot).

Table~\ref{tab:datastats} presents statistical information about the number of commits per project, the number of authors per project, and the projects' age in days. 
These statistics are indicative of the diversity of our dataset, comprised of well-maintained and active open-source Javascript projects. 
\diego{Given that we have an unconventional selection criteria, I think we should show better the distribution of our dataset on some metrics - we used to have that but removed to reduce the number of pages. This would give a more detailed view on the projects we have considered in our analysis as opposed to the table.}


%From this set of candidates we further excluded 569 project that do not contain any package.json file and 413 projects were 
%
%Our selection criteria filtered a total 2,360 projects.
%Based on the reasons expressed above, we decided to clone all repositories locally. We excluded 144 projects which were forks and successfully cloned 2,128 repositories. We excluded 569 projects that did not have a package.json file and 413 projects were removed because had no runtime dependencies in the package.json file. 

%\begin{table*}
%  \caption{Relevant statistical information about our dataset(REDONE)}
%  \label{tab:datastats}
%  \begin{tabular}{l|l|l|l|l|l|l|l}
%    \toprule
%    Criteria & Total & Average & 1st Quartile & Median & 3rd Quartile & Min & Max\\
%    \midrule
%    Commits & 1541504 & 1345 & 237 & 555 & 1479 & 17 & 54548\\
%    Authors & 29400 & 32 & 14 & 21 & 33 & 10 & 420\\
%    Project Age (days) & - & 901 & 248 & 742 & 1354 & 0 & 3626\\
%  \bottomrule
%\end{tabular}
%\end{table*}

\begin{table}
	\centering
	\caption{Relevant statistical information about our dataset.}
	\label{tab:datastats}
	\input{tables/datastats}
\end{table}

%\begin{figure*}[tbh]
%  \begin{subfigure}[b]{0.33\textwidth}
%    \includegraphics[width=\textwidth]{figures/dist_age.pdf}
%    \caption{}
%    \label{fig:1}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.33\textwidth}
%    \includegraphics[width=\textwidth]{figures/dist_commits.pdf}
%    \caption{}
%    \label{fig:2}
%  \end{subfigure}
%  %
%    \begin{subfigure}[b]{0.33\textwidth}
%    \includegraphics[width=\textwidth]{figures/dist_authors.pdf}
%    \caption{}
%    \label{fig:3}
%  \end{subfigure}
%
%\caption{Distribution of age, commits, and authors in the dataset}
%\label{fig:data_dist}
%\end{figure*}

\section{Smell Detection}
\label{sec:smell-detection}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/methodology.png}
  \caption{Methodology for conducting the study.} \abbas{remove figure and references}
  \label{fig:methodology}
%  \Description{methodology}
\end{figure}

We present our methodology in Figure~\ref{fig:methodology}. 
Since we are aiming at analyzing a large dataset of Javascript projects, most of our analyses is automated using a tool we developed specifically for this purpose. 

\abbas{not all smells are regex, some are based on finding a file ans oem on external tools}
\textbf{Identifying dependency smells.}
For each project in our dataset, we parse the package.json file and their related commits and commit diffs. The parser is a prominent part of our methodology because the plain textual diffs are not useful for automated analysis and they can be error-prone. We first parse the package.json file in the latest snapshot of the project and store all dependency profiles in a structured SQL database. These dependency profiles can be queried to obtain information such as the name, version constraint and existing smells.
Many of the existing smells are identified using regex rules on the version constraints.

%This database can be queried to obtain these dependency profiles, containing 
%
%to obtain any information relevant to the dependencies such as the type, number, name, version constraint, and existing smells. 

\textbf{Analysing dependency smells over time.}
Since we want to investigate the evolution of dependency smells over project history, we need to gather the historical information.
We first use \texttt{git log} to identify the commits that modify the package.json file. We then run a large contextual \texttt{git diff} on those commits, i.e., diffs that also include unchanged lines, to properly parse the entire JSON dependency object into a SQL database.
%The parse the result into a similar SQL database. 
%The reason we need a large context for the diffs is because in order to properly parse the JSON dependency object inside package.json, we need to also have the unmodified lines to create a so-called snapshot of the package.json at that time. 
Aside from the dependency profile, this change history database captures commit-relevant information (e.g., commit message, commit date, etc.) needed to investigate the evolution of dependency smells. 
Particularly, this database also contains added, removed, and modified dependencies inside the commits.
Differentiating between these operations are important because we do not want to flag a smells as fixed, due to the removal of the dependency. 
We apply the same regex rules on the new and old version constraint of a modified dependency to determine if a dependency smell is introduced or fixed.



%This change history database captures all of the previously mentioned information, along with commit-relevant information such as commit ID, commit date, commit message, author name, and added/removed/modified dependencies. The modified dependencies refers to those that remained between the commits (were not removed or changed) but experienced a change in their version constraint. We apply the same regex rules on the new and old version constraint of a modified dependency to determine if a dependency smell is introduced or fixed.
% 
%\diego{How? Since this is the core of our methodology, we may want to add more details on what kind of libraries or techniques we use.}
%Thus, for each commit in a project's history, we know (and can query) exactly when the commit was made, who made it, which runtime dependency packages were added/removed/changed, which dependency constraints were added/removed/changed, and which smell (if any) exists in each constraint. 


==> tables/initial_survey.tex <==
%\multirow{4}{*}{\shortstack{Restrictive \\Constraint}} 

\newcommand{\colsize}{1.4cm}
\newcommand{\tablequote}[1]{\textit{#1}}
\newcommand{\tablestm}[1]{\textbf{#1}}
\newcommand{\pro}{$+$}
\newcommand{\con}{$-$}
\begin{tabular}{p{2cm}|p{6.5cm}|p{6.5cm}|p{1cm}}
		\toprule
		
		
		\multirow{2}{\colsize}{Smell / Approach}  
		& \multirow{2}{*}{Statement}
		& Second qualitative survey results
		& \multirow{2}{*}{Overall}\\ %[4ex] 
		%\cline{1-2}		
		
		
		&  & \\
		\cmidrule{1-2} 
		\cmidrule{4-4} 

		
		% PINNED DEPENDENCY
		\multirow{8}{\colsize}{Pinned Dependency}  
		  & \tablestm{\con~Increases bugs and vulnerabilities over time}  & & 4.1
		    \\  %\cline{2-2}
			& & \\  %\cline{2-2}
		   & \tablestm{\con~Increases installation size} & & 3.8
		   \\
			& & \\  %\cline{2-2}
		   & \tablestm{\con~Creates extra overhead for manually updating} & & 3.5
		   \\  %\cline{2-2}
		& & \\  %\cline{2-2}
		   & \tablestm{\pro~Drastically reduces breaking changes} & & 3.2
		   
		   \\  \cline{4-4}
   		\cmidrule{1-2}
   		%[3ex] %\cline{1-2}
   		
   		% URL DEPENDENCY
   		\multirow{8}{\colsize}{URL Dependency}
		& \tablestm{\con~Can cause dependency breakage (link-removal)}  & & 4.6
		\\
		&  &\\  %\cline{2-2}
		  & \tablestm{\con~Increases security risk and bugs}
		  
		  &  \hspace{-0.1cm}
		  \raisebox{-.712\height}[0pt][0pt]{\includegraphics[height=49\normalbaselineskip]{figures/chart.pdf}} & 4.2 
		  \\ %[3ex] %\cline{2-2}
		  & \tablestm{\pro~Useful for non-\npm packages and custom forks}  & & 3.8
		 		  \\
		  & &\\   %\cline{2-2}
		  & \tablestm{\pro~Useful for getting latest fixes not yet published}   & & 2.6
		  		  \\
		  &   &\\ 
		  \cline{4-4}
		   \cmidrule{1-2}
   		
   		
   		% RESTRICTIVE CONSTRAINT
   		 \multirow{4}{\colsize}{Restrictive Constraint}
		 & \tablestm{\pro~Significantly reduces breaking changes}   & & 3.3
		 \\
		 & & \\
		 & \tablestm{\pro~Allows for all important security and bug fixes}  & & 2.3
		 \\
		 & & \\ 
		 \cline{4-4}
   		\cmidrule{1-2} 
  		
  		
  		% PERMISSIVE CONSTRAINT
  		\multirow{4}{\colsize}{Permissive Constraint}
  		 & \tablestm{\con~It is sure to lead to a breaking change}   & & 4.6
  		 \\
  		 & &\\  %\cline{2-2}
   		 & \tablestm{\pro~Makes dependencies easier to manage}  & & 2.2
   		 \\
   		 & 	&\\ 
   		\cline{4-4}
   		 \cmidrule{1-2}
   		
   		
   		% PACKAGE LOCK
   		\multirow{6}{\colsize}{Package Lock}  		
   		& \tablestm{\pro~The best way to ensure consistent installations}   & & 4.9
   		\\
   		& &\\ % [3ex]\cline{2-2}
   		& \tablestm{\pro~Provides a historical snapshots of dependencies}   & & 4.5
   		\\
   		& &\\ % [3ex]\cline{2-2}
  		& \tablestm{\con~Only useful for applications not packages}  & & 2.1
  		\\
  		& &\\
  		\cline{4-4}
  		\cmidrule{1-2}
   		
   		
   		% UNUSED DEPENDENCY
   		 \multirow{4}{\colsize}{Unused Dependency}
   		 & \tablestm{\con~It will cause an extraneous installation of a dependency and waste storage memory}   & & 4.1
   		 \\
   		 & \tablestm{\con~The mismatch between declared and used dependencies confuses users}    & & 3.8
   		 \\
   		 \cline{4-4}
   		 \cmidrule{1-2}
   		
   		
   		% MISSING DEPENDENCY
   		 \multirow{4}{\colsize}{Missing Dependency}
   		 & \tablestm{\con~It will cause unexpected runtime errors}   & & 4.4
		\\
   		 & &  \\ %[3ex]\cline{2-2}
   		 & \tablestm{\con~The mismatch between declared and used dependencies confuses users}   & & 3.9
   		 \\\cline{4-4}
   		\cmidrule{1-2}
   		
   		
   		\multirow{4}{\colsize}{SemVer Compliant}
   		& \tablestm{\pro~Ensures I receive necessary security and bug fixes}   & & 3.9
   		\\
   		& \tablestm{\pro~Ensures I don't experience breaking changes}   & & 3.6
   		\\
   		& &\\
   		
		\bottomrule
	\end{tabular}
